Rao-Blackwellized Markov chain Monte Carlo Light Transport

In light transport simulation, Markov chain Monte Carlo methods are particularly effective at exploring regions with complex lighting characteristics. However, estimator variance is a central concern across Monte Carlo methods in general. In light transport, high variance directly manifests as increased noise or, equivalently, longer rendering times at fixed image quality. Variance reduction techniques based on Rao-Blackwellization have proven particularly effective. In practice, however, the RB approach traditionally used in light transport, waste-recycling, can yield little to no measurable variance reduction, a fact we empirically confirm in this work. Motivated by this lack of effective variance reduction, we introduce a novel RB technique for the general-purpose Metropolis-Hastings algorithm that is computationally efficient and achieves substantial variance reduction. We show that this method consistently outperforms waste-recycling in terms of both variance reduction and convergence speed. Building on this result, we adapt the proposed RB approach to the recently introduced general-purpose Jump Restore algorithm, where it similarly achieves substantial variance reduction and accelerated convergence. Through extensive experiments in light transport simulation, we demonstrate that our \gls{rb} technique significantly outperforms the traditional approaches for both MH-based light transport algorithms and Jump Restore Light Transport, under both equal-time and equal-sample-count comparisons.

==> figures/bathroom.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

\pgfmathsetmacro\width{1024}
\pgfmathsetmacro\height{576}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{bathroom}
\newcommand\firstmethod{metropolis}
\newcommand\secondmethod{metropolis_vanilla}
\newcommand\thirdmethod{metropolis_waste_recycling}
\newcommand\firstmethoddisplaynamea{Metropolis}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{Metropolis}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{Metropolis}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\newcommand\fourthmethod{Metropolis\_Restore}
\newcommand\fifthmethod{Metropolis\_Restore_vanilla}
\newcommand\sixthmethod{Metropolis\_Restore_waste_recycling}
\newcommand\fourthmethoddisplaynamea{Metropolis Restore}
\newcommand\fourthmethoddisplaynameb{\vphantom|}
\newcommand\fifthmethoddisplaynamea{Metropolis Restore}
\newcommand\fifthmethoddisplaynameb{Vanilla (Ours)}
\newcommand\sixthmethoddisplaynamea{Metropolis Restore}
\newcommand\sixthmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.65}
\pgfmathsetmacro\firstcropymin{.3}
\pgfmathsetmacro\secondcropxmin{0}
\pgfmathsetmacro\secondcropymin{0}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}
\pgfmathsetmacro\thirdcropxmin{.65}
\pgfmathsetmacro\thirdcropymin{.3}
\pgfmathsetmacro\fourthcropxmin{0}
\pgfmathsetmacro\fourthcropymin{0}
\newcommand\thirdcropcolor{red}
\newcommand\fourthcropcolor{blue}

\newcommand{\SplitLeftTwoImages}[2]{
    \begin{scope}
       \clip (0, 0) -- (.7 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle ( \aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.7 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#2.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.3 * \aspectratio, 1) -- (.7 * \aspectratio, 0);
   \end{scope}
}

\newcommand{\SplitRightTwoImages}[2]{
    \begin{scope}
       \clip (0, 0) -- (.3 * \aspectratio, 0) -- (.7 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle ( \aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.3 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#2.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.3 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene_\firstmethod_xx}{\scene_\secondmethod_xx}{\scene_\thirdmethod_xx}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene_\firstmethod_xx}{\scene_\secondmethod_xx}{\scene_\thirdmethod_xx}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\fourthmethoddisplaynamea}{\fourthmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\fifthmethoddisplaynamea}{\fifthmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\sixthmethoddisplaynamea}{\sixthmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\firstmethod_xx}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\secondmethod_xx}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\thirdmethod_xx}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\secondmethod_xx}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\fourthmethod_xx}\thirdcropxmin\thirdcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\fifthmethod_xx}\thirdcropxmin\thirdcropymin\croplength{\thirdcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\sixthmethod_xx}\fourthcropxmin\fourthcropymin\croplength{\fourthcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\fifthmethod_xx}\fourthcropxmin\fourthcropymin\croplength{\fourthcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\fourthmethoddisplaynamea}{\fourthmethoddisplaynameb} & \TableMethodLabel{\fifthmethoddisplaynamea}{\fifthmethoddisplaynameb} & \TableMethodLabel{\sixthmethoddisplaynamea}{\sixthmethoddisplaynameb} & \TableMethodLabel{\fifthmethoddisplaynamea}{\fifthmethoddisplaynameb}
\end{tabularx}


==> figures/bathroom2/hmc.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

\pgfmathsetmacro\width{1024}
\pgfmathsetmacro\height{576}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{bathroom2}
\newcommand\firstmethod{HMC}
\newcommand\secondmethod{HMC\_Vanilla\_Ours}
\newcommand\thirdmethod{HMC\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{HMC}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{HMC}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{HMC}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.2}
\pgfmathsetmacro\firstcropymin{.2}
\pgfmathsetmacro\secondcropxmin{.35}
\pgfmathsetmacro\secondcropymin{.12}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/bathroom2/hmc_restore.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

\pgfmathsetmacro\width{1024}
\pgfmathsetmacro\height{576}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{bathroom2}
\newcommand\firstmethod{HMC\_Restore}
\newcommand\secondmethod{HMC\_Restore\_Vanilla\_Ours}
\newcommand\thirdmethod{HMC\_Restore\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{HMC Restore}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{HMC Restore}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{HMC Restore}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.2}
\pgfmathsetmacro\firstcropymin{.2}
\pgfmathsetmacro\secondcropxmin{.35}
\pgfmathsetmacro\secondcropymin{.12}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/bathroom2/mala.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

\pgfmathsetmacro\width{1024}
\pgfmathsetmacro\height{576}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{bathroom2}
\newcommand\firstmethod{MALA}
\newcommand\secondmethod{MALA\_Vanilla\_Ours}
\newcommand\thirdmethod{MALA\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{MALA}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{MALA}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{MALA}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.2}
\pgfmathsetmacro\firstcropymin{.2}
\pgfmathsetmacro\secondcropxmin{.35}
\pgfmathsetmacro\secondcropymin{.12}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/bathroom2/mala_restore.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

\pgfmathsetmacro\width{1024}
\pgfmathsetmacro\height{576}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{bathroom2}
\newcommand\firstmethod{MALA\_Restore}
\newcommand\secondmethod{MALA\_Restore\_Vanilla\_Ours}
\newcommand\thirdmethod{MALA\_Restore\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{MALA Restore}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{MALA Restore}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{MALA Restore}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.2}
\pgfmathsetmacro\firstcropymin{.2}
\pgfmathsetmacro\secondcropxmin{.35}
\pgfmathsetmacro\secondcropymin{.12}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/bathroom2/metropolis.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

\pgfmathsetmacro\width{1024}
\pgfmathsetmacro\height{576}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{bathroom2}
\newcommand\firstmethod{Metropolis}
\newcommand\secondmethod{Metropolis\_Vanilla\_Ours}
\newcommand\thirdmethod{Metropolis\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{Metropolis}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{Metropolis}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{Metropolis}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.2}
\pgfmathsetmacro\firstcropymin{.2}
\pgfmathsetmacro\secondcropxmin{.35}
\pgfmathsetmacro\secondcropymin{.12}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/bathroom2/metropolis_restore.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

\pgfmathsetmacro\width{1024}
\pgfmathsetmacro\height{576}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{bathroom2}
\newcommand\firstmethod{Metropolis\_Restore}
\newcommand\secondmethod{Metropolis\_Restore\_Vanilla\_Ours}
\newcommand\thirdmethod{Metropolis\_Restore\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{Metropolis Restore}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{Metropolis Restore}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{Metropolis Restore}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.2}
\pgfmathsetmacro\firstcropymin{.2}
\pgfmathsetmacro\secondcropxmin{.35}
\pgfmathsetmacro\secondcropymin{.12}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/glass_of_water/metropolis.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{1280}
\pgfmathsetmacro\height{720}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{glass_of_water}
\newcommand\firstmethod{Metropolis}
\newcommand\secondmethod{Metropolis\_Vanilla\_Ours}
\newcommand\thirdmethod{Metropolis\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{Metropolis}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{Metropolis}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{Metropolis}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.275}
\pgfmathsetmacro\firstcropymin{.025}
\pgfmathsetmacro\secondcropxmin{.75}
\pgfmathsetmacro\secondcropymin{.125}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/glass_of_water/metropolis_restore.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{1280}
\pgfmathsetmacro\height{720}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{glass_of_water}
\newcommand\firstmethod{Metropolis\_Restore}
\newcommand\secondmethod{Metropolis\_Restore\_Vanilla\_Ours}
\newcommand\thirdmethod{Metropolis\_Restore\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{Metropolis Restore}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{Metropolis Restore}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{Metropolis Restore}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.275}
\pgfmathsetmacro\firstcropymin{.025}
\pgfmathsetmacro\secondcropxmin{.75}
\pgfmathsetmacro\secondcropymin{.125}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/hmc_pool.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

\pgfmathsetmacro\width{1024}
\pgfmathsetmacro\height{768}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{pool}
\newcommand\firstmethod{hmc}
\newcommand\secondmethod{hmc_vanilla}
\newcommand\thirdmethod{hmc_waste_recycling}
\newcommand\firstmethoddisplaynamea{H²MC}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{H²MC}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{H²MC}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\newcommand\fourthmethod{HMC\_Restore}
\newcommand\fifthmethod{HMC\_Restore_vanilla}
\newcommand\sixthmethod{HMC\_Restore_waste_recycling}
\newcommand\fourthmethoddisplaynamea{H²MC Restore}
\newcommand\fourthmethoddisplaynameb{\vphantom|}
\newcommand\fifthmethoddisplaynamea{H²MC Restore}
\newcommand\fifthmethoddisplaynameb{Vanilla (Ours)}
\newcommand\sixthmethoddisplaynamea{H²MC Restore}
\newcommand\sixthmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.65}
\pgfmathsetmacro\firstcropymin{.3}
\pgfmathsetmacro\secondcropxmin{0}
\pgfmathsetmacro\secondcropymin{0}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}
\pgfmathsetmacro\thirdcropxmin{.65}
\pgfmathsetmacro\thirdcropymin{.3}
\pgfmathsetmacro\fourthcropxmin{0}
\pgfmathsetmacro\fourthcropymin{0}
\newcommand\thirdcropcolor{red}
\newcommand\fourthcropcolor{blue}

\newcommand{\SplitLeftTwoImages}[2]{
    \begin{scope}
       \clip (0, 0) -- (.7 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle ( \aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.7 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#2.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.3 * \aspectratio, 1) -- (.7 * \aspectratio, 0);
   \end{scope}
}

\newcommand{\SplitRightTwoImages}[2]{
    \begin{scope}
       \clip (0, 0) -- (.3 * \aspectratio, 0) -- (.7 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle ( \aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.3 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#2.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.3 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene_\firstmethod}{\scene_\secondmethod}{\scene_\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene_\firstmethod}{\scene_\secondmethod}{\scene_\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\fourthmethoddisplaynamea}{\fourthmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\fifthmethoddisplaynamea}{\fifthmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\sixthmethoddisplaynamea}{\sixthmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\fourthmethod}\thirdcropxmin\thirdcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\fifthmethod}\thirdcropxmin\thirdcropymin\croplength{\thirdcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\sixthmethod}\fourthcropxmin\fourthcropymin\croplength{\fourthcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\fifthmethod}\fourthcropxmin\fourthcropymin\croplength{\fourthcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\fourthmethoddisplaynamea}{\fourthmethoddisplaynameb} & \TableMethodLabel{\fifthmethoddisplaynamea}{\fifthmethoddisplaynameb} & \TableMethodLabel{\sixthmethoddisplaynamea}{\sixthmethoddisplaynameb} & \TableMethodLabel{\fifthmethoddisplaynamea}{\fifthmethoddisplaynameb}
\end{tabularx}


==> figures/mala_pool.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

\pgfmathsetmacro\width{1024}
\pgfmathsetmacro\height{768}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{pool}
\newcommand\firstmethod{mala}
\newcommand\secondmethod{mala_vanilla}
\newcommand\thirdmethod{mala_waste_recycling}
\newcommand\firstmethoddisplaynamea{MALA}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{MALA}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{MALA}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\newcommand\fourthmethod{MALA\_Restore}
\newcommand\fifthmethod{MALA\_Restore_vanilla}
\newcommand\sixthmethod{MALA\_Restore_waste_recycling}
\newcommand\fourthmethoddisplaynamea{MALA Restore}
\newcommand\fourthmethoddisplaynameb{\vphantom|}
\newcommand\fifthmethoddisplaynamea{MALA Restore}
\newcommand\fifthmethoddisplaynameb{Vanilla (Ours)}
\newcommand\sixthmethoddisplaynamea{MALA Restore}
\newcommand\sixthmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.65}
\pgfmathsetmacro\firstcropymin{.3}
\pgfmathsetmacro\secondcropxmin{0}
\pgfmathsetmacro\secondcropymin{0}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}
\pgfmathsetmacro\thirdcropxmin{.65}
\pgfmathsetmacro\thirdcropymin{.3}
\pgfmathsetmacro\fourthcropxmin{0}
\pgfmathsetmacro\fourthcropymin{0}
\newcommand\thirdcropcolor{red}
\newcommand\fourthcropcolor{blue}

\newcommand{\SplitLeftTwoImages}[2]{
    \begin{scope}
       \clip (0, 0) -- (.7 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle ( \aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.7 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#2.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.3 * \aspectratio, 1) -- (.7 * \aspectratio, 0);
   \end{scope}
}

\newcommand{\SplitRightTwoImages}[2]{
    \begin{scope}
       \clip (0, 0) -- (.3 * \aspectratio, 0) -- (.7 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle ( \aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.3 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#2.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.3 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene_\firstmethod}{\scene_\secondmethod}{\scene_\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene_\firstmethod}{\scene_\secondmethod}{\scene_\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\fourthmethoddisplaynamea}{\fourthmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\fifthmethoddisplaynamea}{\fifthmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\sixthmethoddisplaynamea}{\sixthmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\fourthmethod}\thirdcropxmin\thirdcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\fifthmethod}\thirdcropxmin\thirdcropymin\croplength{\thirdcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\sixthmethod}\fourthcropxmin\fourthcropymin\croplength{\fourthcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\fifthmethod}\fourthcropxmin\fourthcropymin\croplength{\fourthcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\fourthmethoddisplaynamea}{\fourthmethoddisplaynameb} & \TableMethodLabel{\fifthmethoddisplaynamea}{\fifthmethoddisplaynameb} & \TableMethodLabel{\sixthmethoddisplaynamea}{\sixthmethoddisplaynameb} & \TableMethodLabel{\fifthmethoddisplaynamea}{\fifthmethoddisplaynameb}
\end{tabularx}


==> figures/metropolis_pool.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

\pgfmathsetmacro\width{1024}
\pgfmathsetmacro\height{768}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{pool}
\newcommand\firstmethod{metropolis}
\newcommand\secondmethod{metropolis_vanilla}
\newcommand\thirdmethod{metropolis_waste_recycling}
\newcommand\firstmethoddisplaynamea{Metropolis}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{Metropolis}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{Metropolis}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\newcommand\fourthmethod{Metropolis\_Restore}
\newcommand\fifthmethod{Metropolis\_Restore_vanilla}
\newcommand\sixthmethod{Metropolis\_Restore_waste_recycling}
\newcommand\fourthmethoddisplaynamea{Metropolis Restore}
\newcommand\fourthmethoddisplaynameb{\vphantom|}
\newcommand\fifthmethoddisplaynamea{Metropolis Restore}
\newcommand\fifthmethoddisplaynameb{Vanilla (Ours)}
\newcommand\sixthmethoddisplaynamea{Metropolis Restore}
\newcommand\sixthmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.65}
\pgfmathsetmacro\firstcropymin{.3}
\pgfmathsetmacro\secondcropxmin{0}
\pgfmathsetmacro\secondcropymin{0}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}
\pgfmathsetmacro\thirdcropxmin{.65}
\pgfmathsetmacro\thirdcropymin{.3}
\pgfmathsetmacro\fourthcropxmin{0}
\pgfmathsetmacro\fourthcropymin{0}
\newcommand\thirdcropcolor{red}
\newcommand\fourthcropcolor{blue}

\newcommand{\SplitLeftTwoImages}[2]{
    \begin{scope}
       \clip (0, 0) -- (.7 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle ( \aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.7 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#2.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.3 * \aspectratio, 1) -- (.7 * \aspectratio, 0);
   \end{scope}
}

\newcommand{\SplitRightTwoImages}[2]{
    \begin{scope}
       \clip (0, 0) -- (.3 * \aspectratio, 0) -- (.7 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle ( \aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.3 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#2.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.3 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene_\firstmethod}{\scene_\secondmethod}{\scene_\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene_\firstmethod}{\scene_\secondmethod}{\scene_\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\fourthmethoddisplaynamea}{\fourthmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\fifthmethoddisplaynamea}{\fifthmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\sixthmethoddisplaynamea}{\sixthmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\fourthmethod}\thirdcropxmin\thirdcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\fifthmethod}\thirdcropxmin\thirdcropymin\croplength{\thirdcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\sixthmethod}\fourthcropxmin\fourthcropymin\croplength{\fourthcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\fifthmethod}\fourthcropxmin\fourthcropymin\croplength{\fourthcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\fourthmethoddisplaynamea}{\fourthmethoddisplaynameb} & \TableMethodLabel{\fifthmethoddisplaynamea}{\fifthmethoddisplaynameb} & \TableMethodLabel{\sixthmethoddisplaynamea}{\sixthmethoddisplaynameb} & \TableMethodLabel{\fifthmethoddisplaynamea}{\fifthmethoddisplaynameb}
\end{tabularx}


==> figures/pool/hmc.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{834}
\pgfmathsetmacro\height{469}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{pool}
\newcommand\firstmethod{HMC}
\newcommand\secondmethod{HMC\_Vanilla\_Ours}
\newcommand\thirdmethod{HMC\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{HMC}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{HMC}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{HMC}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.5}
\pgfmathsetmacro\firstcropymin{.2}
\pgfmathsetmacro\secondcropxmin{.85}
\pgfmathsetmacro\secondcropymin{.35}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/pool/hmc_restore.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{834}
\pgfmathsetmacro\height{469}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{pool}
\newcommand\firstmethod{HMC\_Restore}
\newcommand\secondmethod{HMC\_Restore\_Vanilla\_Ours}
\newcommand\thirdmethod{HMC\_Restore\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{HMC Restore}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{HMC Restore}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{HMC Restore}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.5}
\pgfmathsetmacro\firstcropymin{.2}
\pgfmathsetmacro\secondcropxmin{.85}
\pgfmathsetmacro\secondcropymin{.35}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/pool/mala.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{834}
\pgfmathsetmacro\height{469}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{pool}
\newcommand\firstmethod{MALA}
\newcommand\secondmethod{MALA\_Vanilla\_Ours}
\newcommand\thirdmethod{MALA\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{MALA}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{MALA}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{MALA}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.5}
\pgfmathsetmacro\firstcropymin{.2}
\pgfmathsetmacro\secondcropxmin{.85}
\pgfmathsetmacro\secondcropymin{.35}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/pool/mala_restore.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{834}
\pgfmathsetmacro\height{469}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{pool}
\newcommand\firstmethod{MALA\_Restore}
\newcommand\secondmethod{MALA\_Restore\_Vanilla\_Ours}
\newcommand\thirdmethod{MALA\_Restore\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{MALA Restore}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{MALA Restore}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{MALA Restore}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.5}
\pgfmathsetmacro\firstcropymin{.2}
\pgfmathsetmacro\secondcropxmin{.85}
\pgfmathsetmacro\secondcropymin{.35}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/pool/metropolis.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{834}
\pgfmathsetmacro\height{469}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{pool}
\newcommand\firstmethod{Metropolis}
\newcommand\secondmethod{Metropolis\_Vanilla\_Ours}
\newcommand\thirdmethod{Metropolis\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{Metropolis}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{Metropolis}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{Metropolis}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.5}
\pgfmathsetmacro\firstcropymin{.2}
\pgfmathsetmacro\secondcropxmin{.85}
\pgfmathsetmacro\secondcropymin{.35}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/pool/metropolis_restore.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{834}
\pgfmathsetmacro\height{469}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{pool}
\newcommand\firstmethod{Metropolis\_Restore}
\newcommand\secondmethod{Metropolis\_Restore\_Vanilla\_Ours}
\newcommand\thirdmethod{Metropolis\_Restore\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{Metropolis Restore}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{Metropolis Restore}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{Metropolis Restore}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.5}
\pgfmathsetmacro\firstcropymin{.2}
\pgfmathsetmacro\secondcropxmin{.85}
\pgfmathsetmacro\secondcropymin{.35}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/torus.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

\pgfmathsetmacro\width{1024}
\pgfmathsetmacro\height{576}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{bathroom}
\newcommand\firstmethod{metropolis}
\newcommand\secondmethod{metropolis_vanilla}
\newcommand\thirdmethod{metropolis_waste_recycling}
\newcommand\firstmethoddisplaynamea{Metropolis}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{Metropolis}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{Metropolis}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\newcommand\fourthmethod{Metropolis\_Restore}
\newcommand\fifthmethod{Metropolis\_Restore_vanilla}
\newcommand\sixthmethod{Metropolis\_Restore_waste_recycling}
\newcommand\fourthmethoddisplaynamea{Metropolis Restore}
\newcommand\fourthmethoddisplaynameb{\vphantom|}
\newcommand\fifthmethoddisplaynamea{Metropolis Restore}
\newcommand\fifthmethoddisplaynameb{Vanilla (Ours)}
\newcommand\sixthmethoddisplaynamea{Metropolis Restore}
\newcommand\sixthmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.65}
\pgfmathsetmacro\firstcropymin{.3}
\pgfmathsetmacro\secondcropxmin{0}
\pgfmathsetmacro\secondcropymin{0}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}
\pgfmathsetmacro\thirdcropxmin{.65}
\pgfmathsetmacro\thirdcropymin{.3}
\pgfmathsetmacro\fourthcropxmin{0}
\pgfmathsetmacro\fourthcropymin{0}
\newcommand\thirdcropcolor{red}
\newcommand\fourthcropcolor{blue}

\newcommand{\SplitLeftTwoImages}[2]{
    \begin{scope}
       \clip (0, 0) -- (.7 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle ( \aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.7 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#2.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.3 * \aspectratio, 1) -- (.7 * \aspectratio, 0);
   \end{scope}
}

\newcommand{\SplitRightTwoImages}[2]{
    \begin{scope}
       \clip (0, 0) -- (.3 * \aspectratio, 0) -- (.7 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle ( \aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.3 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#2.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.3 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene_\firstmethod_xx}{\scene_\secondmethod_xx}{\scene_\thirdmethod_xx}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene_\firstmethod_xx}{\scene_\secondmethod_xx}{\scene_\thirdmethod_xx}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\fourthmethoddisplaynamea}{\fourthmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\fifthmethoddisplaynamea}{\fifthmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\sixthmethoddisplaynamea}{\sixthmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\firstmethod_xx}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\secondmethod_xx}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\thirdmethod_xx}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\secondmethod_xx}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\fourthmethod_xx}\thirdcropxmin\thirdcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\fifthmethod_xx}\thirdcropxmin\thirdcropymin\croplength{\thirdcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\sixthmethod_xx}\fourthcropxmin\fourthcropymin\croplength{\fourthcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene_\fifthmethod_xx}\fourthcropxmin\fourthcropymin\croplength{\fourthcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\fourthmethoddisplaynamea}{\fourthmethoddisplaynameb} & \TableMethodLabel{\fifthmethoddisplaynamea}{\fifthmethoddisplaynameb} & \TableMethodLabel{\sixthmethoddisplaynamea}{\sixthmethoddisplaynameb} & \TableMethodLabel{\fifthmethoddisplaynamea}{\fifthmethoddisplaynameb}
\end{tabularx}


==> figures/torus/hmc.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{685}
\pgfmathsetmacro\height{514}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{torus}
\newcommand\firstmethod{HMC}
\newcommand\secondmethod{HMC\_Restore\_Vanilla\_Ours}
\newcommand\thirdmethod{HMC\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{HMC}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{HMC}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{HMC}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.25}
\pgfmathsetmacro\firstcropymin{.3}
\pgfmathsetmacro\secondcropxmin{.075}
\pgfmathsetmacro\secondcropymin{.25}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin - .05)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin - .05 + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin - .05)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin - .05 + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/torus/hmc_restore.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{685}
\pgfmathsetmacro\height{514}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{torus}
\newcommand\firstmethod{HMC\_Restore}
\newcommand\secondmethod{HMC\_Restore\_Vanilla\_Ours}
\newcommand\thirdmethod{HMC\_Restore\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{HMC Restore}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{HMC Restore}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{HMC Restore}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.25}
\pgfmathsetmacro\firstcropymin{.3}
\pgfmathsetmacro\secondcropxmin{.075}
\pgfmathsetmacro\secondcropymin{.25}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin - .05)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin - .05 + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin - .05)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin - .05 + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/torus/mala.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{685}
\pgfmathsetmacro\height{514}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{torus}
\newcommand\firstmethod{MALA}
\newcommand\secondmethod{MALA\_Restore\_Vanilla\_Ours}
\newcommand\thirdmethod{MALA\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{MALA}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{MALA}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{MALA}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.25}
\pgfmathsetmacro\firstcropymin{.3}
\pgfmathsetmacro\secondcropxmin{.075}
\pgfmathsetmacro\secondcropymin{.25}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin - .05)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin - .05 + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin - .05)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin - .05 + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/torus/mala_restore.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{685}
\pgfmathsetmacro\height{514}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{torus}
\newcommand\firstmethod{MALA\_Restore}
\newcommand\secondmethod{MALA\_Restore\_Vanilla\_Ours}
\newcommand\thirdmethod{MALA\_Restore\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{MALA Restore}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{MALA Restore}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{MALA Restore}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.25}
\pgfmathsetmacro\firstcropymin{.3}
\pgfmathsetmacro\secondcropxmin{.075}
\pgfmathsetmacro\secondcropymin{.25}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin - .05)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin - .05 + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin - .05)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin - .05 + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/torus/metropolis.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{685}
\pgfmathsetmacro\height{514}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{torus}
\newcommand\firstmethod{Metropolis}
\newcommand\secondmethod{Metropolis\_Restore\_Vanilla\_Ours}
\newcommand\thirdmethod{Metropolis\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{Metropolis}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{Metropolis}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{Metropolis}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.25}
\pgfmathsetmacro\firstcropymin{.3}
\pgfmathsetmacro\secondcropxmin{.075}
\pgfmathsetmacro\secondcropymin{.25}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin - .05)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin - .05 + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin - .05)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin - .05 + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/torus/metropolis_restore.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{685}
\pgfmathsetmacro\height{514}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{torus}
\newcommand\firstmethod{Metropolis\_Restore}
\newcommand\secondmethod{Metropolis\_Restore\_Vanilla\_Ours}
\newcommand\thirdmethod{Metropolis\_Restore\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{Metropolis Restore}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{Metropolis Restore}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{Metropolis Restore}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.25}
\pgfmathsetmacro\firstcropymin{.3}
\pgfmathsetmacro\secondcropxmin{.075}
\pgfmathsetmacro\secondcropymin{.25}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin - .05)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin - .05 + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin - .05)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin - .05 + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/veach_ajar/metropolis.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{1280}
\pgfmathsetmacro\height{720}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{veach_ajar}
\newcommand\firstmethod{Metropolis}
\newcommand\secondmethod{Metropolis\_Vanilla\_Ours}
\newcommand\thirdmethod{Metropolis\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{Metropolis}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{Metropolis}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{Metropolis}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.5}
\pgfmathsetmacro\firstcropymin{.25}
\pgfmathsetmacro\secondcropxmin{.75}
\pgfmathsetmacro\secondcropymin{.35}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/veach_ajar/metropolis_new_layout.tex <==
%!TEX root = ../main.tex

% Rotated two-line method label (for right margin of table)
% #1 first line, #2 second line
\newcommand{\RotTableMethodLabel}[2]{%
    \smash{%
        \raisebox{0.5\height}{% optisch zentrieren; bei Bedarf feinjustieren
            \rotatebox[origin = c]{90}{%
                \tiny\begin{tabular}{@{}l@{}}
                    \hspace{.6cm}#1\\[.1ex]
                    \hspace{.6cm}#2
                \end{tabular}%
            }%
        }%
    }%
}


% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{1280}
\pgfmathsetmacro\height{720}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{veach_ajar}
\newcommand\firstmethod{Metropolis}
\newcommand\secondmethod{Metropolis\_Vanilla\_Ours}
\newcommand\thirdmethod{Metropolis\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{Metropolis}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{Metropolis}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{Metropolis}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.5}
\pgfmathsetmacro\firstcropymin{.25}
\pgfmathsetmacro\secondcropxmin{.75}
\pgfmathsetmacro\secondcropymin{.35}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 1.78cm, height = 1.78cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}

\begin{tabularx}{\linewidth}{@{}cc@{}}
    \begin{minipage}[t]{.48\linewidth}
    \vspace{0pt}%
    \begin{tikzpicture}[scale = 5.5]
        \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
        \begin{scope}
            \draw[\firstcropcolor, ultra thick]
            (\aspectratio * \firstcropxmin, \firstcropymin)
            rectangle
            (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
            
            \draw[\secondcropcolor, ultra thick]
            (\aspectratio * \secondcropxmin, \secondcropymin)
            rectangle
            (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
        \end{scope}
        \begin{scope}
            \contourlength{.1em}
            \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
            \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
            \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
        \end{scope}
    \end{tikzpicture}
    \end{minipage}
    &
    \hspace{1.25cm}
    \begin{minipage}[t]{.48\linewidth}
    \vspace{0pt}%
    \begin{tabular}{@{}ccccc@{}}
        % row 1
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\firstmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\firstmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
        \end{tikzpicture}
        &
        \RotTableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \\
        % row 2
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale = 1.78]
          \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
        \end{tikzpicture}
        &
        \RotTableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \\
        % row 3
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\thirdmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\thirdmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
        \end{tikzpicture}
        &
        \RotTableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{tabular}
    \end{minipage}
\end{tabularx}


==> figures/veach_ajar/metropolis_restore.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{1280}
\pgfmathsetmacro\height{720}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{veach_ajar}
\newcommand\firstmethod{Metropolis\_Restore}
\newcommand\secondmethod{Metropolis\_Restore\_Vanilla\_Ours}
\newcommand\thirdmethod{Metropolis\_Restore\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{Metropolis Restore}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{Metropolis Restore}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{Metropolis Restore}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.5}
\pgfmathsetmacro\firstcropymin{.25}
\pgfmathsetmacro\secondcropxmin{.75}
\pgfmathsetmacro\secondcropymin{.35}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/zero_day.tex <==
%!TEX root = ../main.tex

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{685}
\pgfmathsetmacro\height{514}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\system{pbrt4}
\newcommand\scene{bathroom}
\newcommand\firstmethod{metropolis}
\newcommand\secondmethod{metropolis_vanilla}
\newcommand\thirdmethod{metropolis_waste_recycling}
\newcommand\firstmethoddisplayname{Metropolis}
\newcommand\secondmethoddisplayname{Metropolis Vanilla (Ours)}
\newcommand\thirdmethoddisplayname{Metropolis Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
% \pgfmathsetmacro\firstcropxmin{.2}
% \pgfmathsetmacro\firstcropymin{.2}
\pgfmathsetmacro\firstcropxmin{.075}
\pgfmathsetmacro\firstcropymin{.25}
\pgfmathsetmacro\secondcropxmin{.7}
\pgfmathsetmacro\secondcropymin{.4}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}


\newcommand{\SplitLeftTwoImages}[2]{
    \begin{scope}
       \clip (0, 0) -- (.7 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle ( \aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.7 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#2.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.3 * \aspectratio, 1) -- (.7 * \aspectratio, 0);
   \end{scope}
}

\newcommand{\SplitRightTwoImages}[2]{
    \begin{scope}
       \clip (0, 0) -- (.3 * \aspectratio, 0) -- (.7 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle ( \aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.3 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#2.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.3 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle ( \aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle ( \aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}


\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\system/\scene/_\scene_\firstmethod_120}{\system/\scene/_\scene_\secondmethod_120}{\system/\scene/_\scene_\thirdmethod_120}
    % \SplitTwoImages{\system/\scene/_\scene_\firstmethod_120}{\system/\scene/_\scene_\secondmethod_120}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \node[anchor = west] at (0.025, 0.93) {\contour{black}{\textcolor{white}\firstmethoddisplayname}};
        \node[anchor = west] at (.575, 0.93) {\contour{black}{\textcolor{white}\secondmethoddisplayname}};
        \node[anchor = east] at (1.75, 0.93) {\contour{black}{\textcolor{white}\thirdmethoddisplayname}};
        % \node[anchor = east] at (1.75, 0.93) {\contour{black}{\textcolor{white}\secondmethoddisplayname}};
        % \node[anchor = east] at (0.35, 0.93) {\contour{black}{\textcolor{white}\firstmethoddisplayname}};
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\system/\scene/_\scene_\firstmethod_120_error}{\system/\scene/_\scene_\secondmethod_120_error}{\system/\scene/_\scene_\thirdmethod_120_error}
    % \SplitLeftTwoImages{\system/\scene/_\scene_\firstmethod_120_error}{\system/\scene/_\scene_\secondmethod_120_error}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\system/\scene/_\scene_\firstmethod_120}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\system/\scene/_\scene_\secondmethod_120}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\system/\scene/_\scene_\thirdmethod_120}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\system/\scene/_\scene_\secondmethod_120}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\system/\scene/_\scene_\firstmethod_120_error}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\system/\scene/_\scene_\secondmethod_120_error}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\system/\scene/_\scene_\thirdmethod_120_error}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\system/\scene/_\scene_\secondmethod_120_error}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.75mm]
\tiny\firstmethoddisplayname  & \tiny\secondmethoddisplayname & \tiny\thirdmethoddisplayname & \tiny\secondmethoddisplayname & \tiny\firstmethoddisplayname & \tiny\secondmethoddisplayname & ´\tiny\thirdmethoddisplayname & \tiny\secondmethoddisplayname
\end{tabularx}


==> figures/zero_day/metropolis.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{1280}
\pgfmathsetmacro\height{720}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{zero_day}
\newcommand\firstmethod{Metropolis}
\newcommand\secondmethod{Metropolis\_Vanilla\_Ours}
\newcommand\thirdmethod{Metropolis\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{Metropolis}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{Metropolis}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{Metropolis}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.175}
\pgfmathsetmacro\firstcropymin{.7}
\pgfmathsetmacro\secondcropxmin{.44}
\pgfmathsetmacro\secondcropymin{.46}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/zero_day/metropolis_restore.tex <==
%!TEX root = ../main.tex

% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{1280}
\pgfmathsetmacro\height{720}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{zero_day}
\newcommand\firstmethod{Metropolis\_Restore}
\newcommand\secondmethod{Metropolis\_Restore\_Vanilla\_Ours}
\newcommand\thirdmethod{Metropolis\_Restore\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{Metropolis Restore}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{Metropolis Restore}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{Metropolis Restore}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.175}
\pgfmathsetmacro\firstcropymin{.7}
\pgfmathsetmacro\secondcropxmin{.44}
\pgfmathsetmacro\secondcropymin{.46}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 2.15cm, height = 2.15cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}
\begin{tabularx}{\linewidth}{cccccccc}
%
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
    \begin{scope}
        \draw[\firstcropcolor, ultra thick]
        (\aspectratio * \firstcropxmin, \firstcropymin)
        rectangle
        (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        \draw[\secondcropcolor, ultra thick]
        (\aspectratio * \secondcropxmin, \secondcropymin)
        rectangle
        (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
    \begin{scope}
        \contourlength{.1em}
        \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{scope}
\end{tikzpicture}
}
&
\multicolumn{4}{c}{
\begin{tikzpicture}[scale = 5]
    \SplitThreeImages{\scene/\firstmethod-MAPE}{\scene/\secondmethod-MAPE}{\scene/\thirdmethod-MAPE}
    \begin{scope}
        % \draw[\firstcropcolor, ultra thick]
        % (\aspectratio * \firstcropxmin, \firstcropymin)
        % rectangle
        % (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
        
        % \draw[\secondcropcolor, ultra thick]
        % (\aspectratio * \secondcropxmin, \secondcropymin)
        % rectangle
        % (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
    \end{scope}
\end{tikzpicture}
}
\\
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
&
\begin{tikzpicture}[scale = 2.15]
    \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
\end{tikzpicture}
\\[-.25mm]
\TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb} & \TableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb} & \TableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
\end{tabularx}


==> figures/zero_day/metropolis_restore_new_layout.tex <==
%!TEX root = ../main.tex

% Rotated two-line method label (for right margin of table)
% #1 first line, #2 second line
\newcommand{\RotTableMethodLabel}[2]{%
    \smash{%
        \raisebox{0.5\height}{% optisch zentrieren; bei Bedarf feinjustieren
            \rotatebox[origin = c]{90}{%
                \tiny\begin{tabular}{@{}l@{}}
                    \hspace{.6cm}#1\\[.1ex]
                    \hspace{.6cm}#2
                \end{tabular}%
            }%
        }%
    }%
}


% #1 = x position
% #2 = y position
% #3 = anchor
% #3 = first line
% #4 = second line
\newcommand{\MethodLabelAt}[5]{%
  \node[anchor = #3] at (#1, #2) {%
    \shortstack[l]{%
      \contour{black}{\small\textcolor{white}{#4}}\\[-0.2ex]%
      \contour{black}{\small\textcolor{white}{#5}}%
    }%
  };%
}

% Two-line tiny label for tables (left-aligned)
\newcommand{\TableMethodLabel}[2]{%
  \begin{tabular}{@{}l@{}}%
    \tiny #1\\[-0.1ex]%
    \tiny #2%
  \end{tabular}%
}

% \pgfmathsetmacro\width{1024}
% \pgfmathsetmacro\height{768}
\pgfmathsetmacro\width{1280}
\pgfmathsetmacro\height{720}
\pgfmathsetmacro\aspectratio{16 / 9}

\newcommand\scene{zero_day}
\newcommand\firstmethod{Metropolis\_Restore}
\newcommand\secondmethod{Metropolis\_Restore\_Vanilla\_Ours}
\newcommand\thirdmethod{Metropolis\_Restore\_Waste-Recycling}
\newcommand\firstmethoddisplaynamea{Metropolis Restore}
\newcommand\firstmethoddisplaynameb{\vphantom|}
\newcommand\secondmethoddisplaynamea{Metropolis Restore}
\newcommand\secondmethoddisplaynameb{Vanilla (Ours)}
\newcommand\thirdmethoddisplaynamea{Metropolis Restore}
\newcommand\thirdmethoddisplaynameb{Waste-Recycling}

\pgfmathsetmacro\croplength{.12}
\pgfmathsetmacro\firstcropxmin{.175}
\pgfmathsetmacro\firstcropymin{.7}
\pgfmathsetmacro\secondcropxmin{.44}
\pgfmathsetmacro\secondcropymin{.46}
\newcommand\firstcropcolor{red}
\newcommand\secondcropcolor{blue}

\newcommand{\SplitThreeImages}[3]{
    \begin{scope}
       \clip (0, 0) -- (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1) -- (0, 1) -- cycle;
        \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
    \begin{scope}
       \clip (.2 * \aspectratio, 0) -- (0.6 * \aspectratio, 0) -- (0.7 * \aspectratio, 1) -- (0.3 * \aspectratio, 1) -- cycle;
        \path[fill overzoom image = results/#2.jpg] (0, 0) rectangle (\aspectratio, 1);
    \end{scope}
   \begin{scope}
       \clip (.6 * \aspectratio, 0) -- (\aspectratio, 0) -- (\aspectratio, 1) -- (0.7 * \aspectratio, 1) -- cycle;
       \path[fill overzoom image = results/#3.jpg] (0,0) rectangle (\aspectratio, 1);
   \end{scope}
   \begin{scope}
        \draw[black, thick] (0, 0) rectangle (\aspectratio, 1);
        \draw[draw=black,thick] (.2 * \aspectratio, 0) -- (.3 * \aspectratio, 1);
        \draw[draw=black,thick] (.6 * \aspectratio, 0) -- (.7 * \aspectratio, 1);
   \end{scope}
}

%   - #1: scene name (without extension; image is results/#1.jpg)
%   - #2: crop x (normalized, 0–1; 0=left)
%   - #3: crop y (normalized, 0–1; 0=bottom; note: image origin is lower left)
%   - #4: crop length (normalized)
%   - #5: color (for drawing the outline)
\newcommand{\CropImage}[5]{%
    \begingroup
        % Convert normalized crop to pixel values
        \pgfmathsetmacro\length{#4 * \width}
        \pgfmathsetmacro\xminval{#2 * \width}
        \pgfmathsetmacro\xmaxval{#2 * \width + \length}
        \pgfmathsetmacro\yminval{(1 - #3) * \height - \length}
        \pgfmathsetmacro\ymaxval{(1 - #3) * \height}

        \begin{scope}
            % Use fill with a rectangle, not a node
            \path[fill overzoom image = results/#1.jpg] (0, 0) rectangle (1, 1);
            % Now clip to viewport
            \clip (0, 0) rectangle (1, 1);
            \begin{scope}[xscale = 1, yscale = 1]
                \pgfmathsetmacro{\trimleft}{\xminval}
                \pgfmathsetmacro{\trimbottom}{\height - \ymaxval}  % Flip y-axis because trim starts from top-left
                \pgfmathsetmacro{\trimright}{\width - \xmaxval}
                \pgfmathsetmacro{\trimtop}{\yminval}
                
                \node at (0.5,0.5) {%
                    \includegraphics[
                        width = 1.78cm, height = 1.78cm,
                        trim = {\trimleft bp} {\trimbottom bp} {\trimright bp} {\trimtop bp},
                        clip
                    ]{results/#1.jpg}%
                };
            \end{scope}
        \end{scope}

        \begin{scope}
            \draw[#5, thick] (0, 0) rectangle (1, 1);
        \end{scope}
    \endgroup
}

\def\arraystretch{.5}
\setlength\tabcolsep{1pt}

\begin{tabularx}{\linewidth}{@{}cc@{}}
    \begin{minipage}[t]{.48\linewidth}
    \vspace{0pt}%
    \begin{tikzpicture}[scale = 5.5]
        \SplitThreeImages{\scene/\firstmethod}{\scene/\secondmethod}{\scene/\thirdmethod}
        \begin{scope}
            \draw[\firstcropcolor, ultra thick]
            (\aspectratio * \firstcropxmin, \firstcropymin)
            rectangle
            (\aspectratio * \firstcropxmin + \aspectratio * \croplength, \firstcropymin + \aspectratio * \croplength);
            
            \draw[\secondcropcolor, ultra thick]
            (\aspectratio * \secondcropxmin, \secondcropymin)
            rectangle
            (\aspectratio * \secondcropxmin + \aspectratio * \croplength, \secondcropymin + \aspectratio * \croplength);
        \end{scope}
        \begin{scope}
            \contourlength{.1em}
            \MethodLabelAt{.025}{.9}{west}{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
            \MethodLabelAt{.6}{.9}{west}{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
            \MethodLabelAt{1.26}{.9}{west}{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
        \end{scope}
    \end{tikzpicture}
    \end{minipage}
    &
    \hspace{1.25cm}
    \begin{minipage}[t]{.48\linewidth}
    \vspace{0pt}%
    \begin{tabular}{@{}ccccc@{}}
        % row 1
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\firstmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\firstmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\firstmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\firstmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
        \end{tikzpicture}
        &
        \RotTableMethodLabel{\firstmethoddisplaynamea}{\firstmethoddisplaynameb}
        \\
        % row 2
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\secondmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale = 1.78]
          \CropImage{\scene/\secondmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\secondmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\secondmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
        \end{tikzpicture}
        &
        \RotTableMethodLabel{\secondmethoddisplaynamea}{\secondmethoddisplaynameb}
        \\
        % row 3
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\thirdmethod}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\thirdmethod-MAPE}\firstcropxmin\firstcropymin\croplength{\firstcropcolor}
        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\thirdmethod}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
        \end{tikzpicture}
        &
        \begin{tikzpicture}[scale = 1.78]
            \CropImage{\scene/\thirdmethod-MAPE}\secondcropxmin\secondcropymin\croplength{\secondcropcolor}
        \end{tikzpicture}
        &
        \RotTableMethodLabel{\thirdmethoddisplaynamea}{\thirdmethoddisplaynameb}
    \end{tabular}
    \end{minipage}
\end{tabularx}


==> plots/c0.tex <==
\begin{tikzpicture}%[scale = .48]
    \begin{axis}[
        title = {\textsc{Country Kitchen}},
        grid = major,
        xlabel = {\Gls{spp}},
        ylabel = {\Gls{mse}},
        ymode = log,
        xmin = 0,
        xmax = 256,
        log ticks with fixed point,
        xtick = {32, 64, 128, 256},
        xticklabels = {$32$, $64$, $128$, $256$},
        ytick = {.1, .25, .5, 1},
        yticklabels = {$.1$, $.25$, $.5$, $1$},
        yminorticks = false,
        tick align = outside,
    ]
        \addplot[smooth, thick, red, no markers] table[x index = 0, y index = 2, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla_1.log};
        \addplot[smooth, thick, green, no markers] table[x index = 0, y index = 2, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla_0.1.log};
        \addplot[smooth, thick, blue, no markers] table[x index = 0, y index = 2, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla_0.01.log};
        \addplot[smooth, thick, magenta, no markers] table[x index = 0, y index = 2, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla_0.001.log};
        \addplot[smooth, thick, cyan, no markers] table[x index = 0, y index = 2, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla_0.0005.log};
        \addplot[smooth, thick, orange, no markers] table[x index = 0, y index = 2, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla_0.0001.log};
        \addlegendentry{1}
        \addlegendentry{.1}
        \addlegendentry{.01}
        \addlegendentry{.001}
        \addlegendentry{.0005}
        \addlegendentry{.0001}
    \end{axis}
\end{tikzpicture}
\clearpage
\begin{tikzpicture}%[scale = .48]
    \begin{axis}[
        title = {\textsc{Country Kitchen}},
        grid = major,
        xlabel = {Computation time in seconds},
        ylabel = {\Gls{mse}},
        ymode = log,
        xmin = 0,
        xmax = 20,
        log ticks with fixed point,
        xtick = {5, 10, 15, 20},
        xticklabels = {$5$, $10$, $15$, $20$},
        ytick = {.1, .25, .5, 1},
        yticklabels = {$.1$, $.25$, $.5$, $1$},
        yminorticks = false,
        tick align = outside,
    ]
        \addplot[smooth, thick, red, no markers] table[x index = 1, y index = 2, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla_1.log};
        \addplot[smooth, thick, green, no markers] table[x index = 1, y index = 2, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla_0.1.log};
        \addplot[smooth, thick, blue, no markers] table[x index = 1, y index = 2, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla_0.01.log};
        \addplot[smooth, thick, magenta, no markers] table[x index = 1, y index = 2, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla_0.001.log};
        \addplot[smooth, thick, cyan, no markers] table[x index = 1, y index = 2, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla_0.0005.log};
        \addplot[smooth, thick, orange, no markers] table[x index = 1, y index = 2, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla_0.0001.log};
        \addlegendentry{1}
        \addlegendentry{.1}
        \addlegendentry{.01}
        \addlegendentry{.001}
        \addlegendentry{.0005}
        \addlegendentry{.0001}
    \end{axis}
\end{tikzpicture}

\clearpage

\begin{tikzpicture}%[scale = .48]
    \begin{axis}[
        title = {\textsc{Glass of Water}},
        grid = major,
        xlabel = {\Gls{spp}},
        ylabel = {\Gls{mse}},
        ymode = log,
        xmin = 0,
        xmax = 256,
        log ticks with fixed point,
        xtick = {32, 64, 128, 256},
        xticklabels = {$32$, $64$, $128$, $256$},
        ytick = {.1, .25, .5, 1},
        yticklabels = {$.1$, $.25$, $.5$, $1$},
        yminorticks = false,
        tick align = outside,
    ]
        \addplot[smooth, thick, red, no markers] table[x index = 0, y index = 2, col sep = tab] {results/glass_of_water_Metropolis\_Restore_vanilla_1.log};
        \addplot[smooth, thick, green, no markers] table[x index = 0, y index = 2, col sep = tab] {results/glass_of_water_Metropolis\_Restore_vanilla_0.1.log};
        \addplot[smooth, thick, blue, no markers] table[x index = 0, y index = 2, col sep = tab] {results/glass_of_water_Metropolis\_Restore_vanilla_0.01.log};
        \addplot[smooth, thick, magenta, no markers] table[x index = 0, y index = 2, col sep = tab] {results/glass_of_water_Metropolis\_Restore_vanilla_0.001.log};
        \addplot[smooth, thick, cyan, no markers] table[x index = 0, y index = 2, col sep = tab] {results/glass_of_water_Metropolis\_Restore_vanilla_0.0005.log};
        \addplot[smooth, thick, orange, no markers] table[x index = 0, y index = 2, col sep = tab] {results/glass_of_water_Metropolis\_Restore_vanilla_0.0001.log};
        \addlegendentry{1}
        \addlegendentry{.1}
        \addlegendentry{.01}
        \addlegendentry{.001}
        \addlegendentry{.0005}
        \addlegendentry{.0001}
    \end{axis}
\end{tikzpicture}
\clearpage
\begin{tikzpicture}%[scale = .48]
    \begin{axis}[
        title = {\textsc{Glass of Water}},
        grid = major,
        xlabel = {Computation time in seconds},
        ylabel = {\Gls{mse}},
        ymode = log,
        xmin = 0,
        xmax = 20,
        log ticks with fixed point,
        xtick = {5, 10, 15, 20},
        xticklabels = {$5$, $10$, $15$, $20$},
        ytick = {.1, .25, .5, 1},
        yticklabels = {$.1$, $.25$, $.5$, $1$},
        yminorticks = false,
        tick align = outside,
    ]
        \addplot[smooth, thick, red, no markers] table[x index = 1, y index = 2, col sep = tab] {results/glass_of_water_Metropolis\_Restore_vanilla_1.log};
        \addplot[smooth, thick, green, no markers] table[x index = 1, y index = 2, col sep = tab] {results/glass_of_water_Metropolis\_Restore_vanilla_0.1.log};
        \addplot[smooth, thick, blue, no markers] table[x index = 1, y index = 2, col sep = tab] {results/glass_of_water_Metropolis\_Restore_vanilla_0.01.log};
        \addplot[smooth, thick, magenta, no markers] table[x index = 1, y index = 2, col sep = tab] {results/glass_of_water_Metropolis\_Restore_vanilla_0.001.log};
        \addplot[smooth, thick, cyan, no markers] table[x index = 1, y index = 2, col sep = tab] {results/glass_of_water_Metropolis\_Restore_vanilla_0.0005.log};
        \addplot[smooth, thick, orange, no markers] table[x index = 1, y index = 2, col sep = tab] {results/glass_of_water_Metropolis\_Restore_vanilla_0.0001.log};
        \addlegendentry{1}
        \addlegendentry{.1}
        \addlegendentry{.01}
        \addlegendentry{.001}
        \addlegendentry{.0005}
        \addlegendentry{.0001}
    \end{axis}
\end{tikzpicture}


==> plots/error_pool_torus.tex <==
\centering
\begin{subfigure}[t]{.2\textwidth}
    \centering
    \begin{tikzpicture}[scale = .48]
        \begin{axis}[
            title = {\textsc{Swimming Pool}},
            title style = {yshift = -1.5ex},
            grid = major,
            xlabel = {Rendering time in seconds},
            ylabel = {\Gls{mse}},
            ylabel style = {yshift = .05cm},
            ymode = log,
            xmin = 1,
            xmax = 60,
            log ticks with fixed point,
            tick align = outside,
            xminorticks = false,
            yminorticks = false,
        ]
            \addplot[smooth, tension = .2, color = black, thick, thick, no markers] table[x index = 1, y index = 2, col sep = tab] {results/pool_mala.txt};
            \addplot[smooth, tension = .2, color = red, thick, no markers] table[x index = 1, y index = 2, col sep = tab] {results/pool_mala_vanilla.txt};
            \addplot[smooth, tension = .2, color = blue, thick, no markers] table[x index = 1, y index = 2, col sep = tab] {results/pool_mala_waste_recycling.txt};
        \end{axis}
    \end{tikzpicture}
\end{subfigure}
\hspace{.5cm}
\begin{subfigure}[t]{.2\textwidth}
    \centering
    \begin{tikzpicture}[scale = .48]
        \begin{axis}[
            title = {\textsc{Swimming Pool}},
            title style = {yshift = -1.5ex},
            grid = major,
            xlabel = {Rendering time in seconds},
            ylabel = {Empirical variance},
            ylabel style = {yshift = .05cm},
            ymode = log,
            xmin = 1,
            xmax = 60,
            log ticks with fixed point,
            tick align = outside,
            xminorticks = false,
            yminorticks = false,
        ]
            \addplot[smooth, tension = .2, color = black, thick, thick, no markers] table[x index = 1, y index = 5, col sep = tab] {results/pool_MALA\_Restore.txt};
            \addplot[smooth, tension = .2, color = red, thick, no markers] table[x index = 1, y index = 5, col sep = tab] {results/pool_MALA\_Restore_vanilla.txt};
            \addplot[smooth, tension = .2, color = blue, thick, no markers] table[x index = 1, y index = 5, col sep = tab] {results/pool_MALA\_Restore_waste_recycling.txt};
        \end{axis}
    \end{tikzpicture}
\end{subfigure}
\hspace{.5cm}
\begin{subfigure}[t]{.2\textwidth}
    \centering
    \begin{tikzpicture}[scale = .48]
        \begin{axis}[
            title = {\textsc{Torus}},
            title style = {yshift = -1.5ex},
            grid = major,
            xlabel = {Rendering time in seconds},
            ylabel = {\Gls{mse}},
            ylabel style = {yshift = .05cm},
            ymode = log,
            xmin = 1,
            xmax = 60,
            log ticks with fixed point,
            tick align = outside,
            xminorticks = false,
            yminorticks = false,
        ]
            \addplot[smooth, tension = .2, color = black!50, thick, thick, thick, no markers] table[x index = 1, y index = 2, col sep = tab] {results/torus_hmc.txt};
            \addplot[smooth, tension = .2, color = orange!90!black, thick, thick, no markers] table[x index = 1, y index = 2, col sep = tab] {results/torus_hmc_vanilla.txt};
            \addplot[smooth, tension = .2, color = teal!80!black, thick, thick, no markers] table[x index = 1, y index = 2, col sep = tab] {results/torus_hmc_waste_recycling.txt};
        \end{axis}
    \end{tikzpicture}
\end{subfigure}
\hspace{.5cm}
\begin{subfigure}[t]{.2\textwidth}
    \centering
    \begin{tikzpicture}[scale = .48]
        \begin{axis}[
            title = {\textsc{Torus}},
            title style = {yshift = -1.5ex},
            grid = major,
            xlabel = {Rendering time in seconds},
            ylabel = {Empirical variance},
            ylabel style = {yshift = .05cm},
            ymode = log,
            xmin = 1,
            xmax = 60,
            log ticks with fixed point,
            tick align = outside,
            xminorticks = false,
            yminorticks = false,
        ]
            \addplot[smooth, tension = .2, color = black!50, thick, thick, thick, no markers] table[x index = 1, y index = 5, col sep = tab] {results/torus_hmc.txt};
            \addplot[smooth, tension = .2, color = orange!90!black, thick, thick, no markers] table[x index = 1, y index = 5, col sep = tab] {results/torus_hmc_vanilla.txt};
            \addplot[smooth, tension = .2, color = teal!80!black, thick, thick, no markers] table[x index = 1, y index = 5, col sep = tab] {results/torus_hmc_waste_recycling.txt};
        \end{axis}
    \end{tikzpicture}
\end{subfigure}
\par\nointerlineskip\vspace{-.7mm}
\begin{tikzpicture}
    \begin{axis}[
        hide axis,
        width = 0pt,
        height = 0pt,
        xmin = 0,
        xmax = 1,
        ymin = 0,
        ymax = 1,
        legend columns = 6,
        legend style = {
            draw = none,
            font = \scriptsize, /tikz/every even column/.append, style = {column sep = .25cm},
        },
        legend image code/.code = {
            \draw[#1, thick] (0cm, 0cm) -- (.35cm, 0cm);
        },
    ]
        \addlegendimage{black, thick}
        \addlegendentry{\gls{mala} Restore}
        \addlegendimage{red, thick}
        \addlegendentry{\gls{mala} Restore Vanilla (Ours)}
        \addlegendimage{blue, thick}
        \addlegendentry{\gls{mala} Restore Waste-Recycling}
        
        \addlegendimage{black!50, thick}
        \addlegendentry{\gls{hmc}}
        \addlegendimage{orange!90!black, thick}
        \addlegendentry{\gls{hmc} Vanilla (Ours)}
        \addlegendimage{teal!80!black, thick}
        \addlegendentry{\gls{hmc} Waste-Recycling}
    \end{axis}
\end{tikzpicture}

==> plots/error_veach_ajar_glass_of_water.tex <==
\centering
\begin{subfigure}[t]{.2\textwidth}
    \centering
    \begin{tikzpicture}[scale = .48]
        \begin{axis}[
            title = {\textsc{Veach, Ajar}},
            title style = {yshift = -1.5ex},
            grid = major,
            xlabel = {Rendering time in seconds},
            ylabel = {\Gls{mse}},
            ylabel style = {yshift = -.05cm},
            ymode = log,
            xmin = 1,
            xmax = 60,
            log ticks with fixed point,
            tick align = outside,
            xminorticks = false,
            yminorticks = false,
        ]
            \addplot[smooth, tension = .2, color = black, thick, thick, no markers] table[x index = 1, y index = 2, col sep = tab] {results/veach_ajar_metropolis.txt};
            \addplot[smooth, tension = .2, color = red, thick, no markers] table[x index = 1, y index = 2, col sep = tab] {results/veach_ajar_metropolis_vanilla.txt};
            \addplot[smooth, tension = .2, color = blue, thick, no markers] table[x index = 1, y index = 2, col sep = tab] {results/veach_ajar_metropolis_waste_recycling.txt};
        \end{axis}
    \end{tikzpicture}
\end{subfigure}
\hspace{.5cm}
\begin{subfigure}[t]{.2\textwidth}
    \centering
    \begin{tikzpicture}[scale = .48]
        \begin{axis}[
            title = {\textsc{Veach, Ajar}},
            title style = {yshift = -1.5ex},
            grid = major,
            xlabel = {Rendering time in seconds},
            ylabel = {Empirical variance},
            ylabel style = {yshift = -.05cm},
            ymode = log,
            xmin = 1,
            xmax = 60,
            log ticks with fixed point,
            tick align = outside,
            xminorticks = false,
            yminorticks = false,
        ]
            \addplot[smooth, tension = .2, color = black, thick, thick, no markers] table[x index = 1, y index = 5, col sep = tab] {results/veach_ajar_metropolis.txt};
            \addplot[smooth, tension = .2, color = red, thick, no markers] table[x index = 1, y index = 5, col sep = tab] {results/veach_ajar_metropolis_vanilla.txt};
            \addplot[smooth, tension = .2, color = blue, thick, no markers] table[x index = 1, y index = 5, col sep = tab] {results/veach_ajar_metropolis_waste_recycling.txt};
        \end{axis}
    \end{tikzpicture}
\end{subfigure}
\hspace{.5cm}
\begin{subfigure}[t]{.2\textwidth}
    \centering
    \begin{tikzpicture}[scale = .48]
        \begin{axis}[
            title = {\textsc{Glass of Water}},
            title style = {yshift = -1.5ex},
            grid = major,
            xlabel = {Rendering time in seconds},
            ylabel = {\Gls{mse}},
            ylabel style = {yshift = -.05cm},
            ymode = log,
            xmin = 1,
            xmax = 60,
            log ticks with fixed point,
            tick align = outside,
            xminorticks = false,
            yminorticks = false,
        ]
            \addplot[smooth, tension = .2, color = black, thick, thick, no markers] table[x index = 1, y index = 2, col sep = tab] {results/glass_of_water_metropolis.txt};
            \addplot[smooth, tension = .2, color = red, thick, no markers] table[x index = 1, y index = 2, col sep = tab] {results/glass_of_water_metropolis_vanilla.txt};
            \addplot[smooth, tension = .2, color = blue, thick, no markers] table[x index = 1, y index = 2, col sep = tab] {results/glass_of_water_metropolis_waste_recycling.txt};
        \end{axis}
    \end{tikzpicture}
\end{subfigure}
\hspace{.5cm}
\begin{subfigure}[t]{.2\textwidth}
    \centering
    \begin{tikzpicture}[scale = .48]
        \begin{axis}[
            title = {\textsc{Glass of Water}},
            title style = {yshift = -1.5ex},
            grid = major,
            xlabel = {Rendering time in seconds},
            ylabel = {Empirical variance},
            ylabel style = {yshift = -.05cm},
            ymode = log,
            xmin = 1,
            xmax = 60,
            log ticks with fixed point,
            tick align = outside,
            xminorticks = false,
            yminorticks = false,
        ]
            \addplot[smooth, tension = .2, color = black, thick, thick, no markers] table[x index = 1, y index = 5, col sep = tab] {results/glass_of_water_metropolis.txt};
            \addplot[smooth, tension = .2, color = red, thick, no markers] table[x index = 1, y index = 5, col sep = tab] {results/glass_of_water_metropolis_vanilla.txt};
            \addplot[smooth, tension = .2, color = blue, thick, no markers] table[x index = 1, y index = 5, col sep = tab] {results/glass_of_water_metropolis_waste_recycling.txt};
        \end{axis}
    \end{tikzpicture}
\end{subfigure}
\par\nointerlineskip\vspace{-.7mm}
\begin{tikzpicture}
    \begin{axis}[
        hide axis,
        width = 0pt,
        height = 0pt,
        xmin = 0,
        xmax = 1,
        ymin = 0,
        ymax = 1,
        legend columns = 6,
        legend style = {
            draw = none,
            font = \scriptsize, /tikz/every even column/.append, style = {column sep = .25cm},
        },
        legend image code/.code = {
            \draw[#1, thick] (0cm, 0cm) -- (.35cm, 0cm);
        },
    ]
        \addlegendimage{black, thick}
        \addlegendentry{\gls{mala} Restore}
        \addlegendimage{red, thick}
        \addlegendentry{\gls{mala} Restore Vanilla (Ours)}
        \addlegendimage{blue, thick}
        \addlegendentry{\gls{mala} Restore Waste-Recycling}
        
        \addlegendimage{black!50, thick}
        \addlegendentry{\gls{hmc}}
        \addlegendimage{orange!90!black, thick}
        \addlegendentry{\gls{hmc} Vanilla (Ours)}
        \addlegendimage{teal!80!black, thick}
        \addlegendentry{\gls{hmc} Waste-Recycling}
    \end{axis}
\end{tikzpicture}

==> plots/kitchen.tex <==
\begin{tikzpicture}%[scale = .48]
    \begin{axis}[
        grid = major,
        %xlabel = {Computation time in seconds},
        ylabel = {Mean absolute error (MAE)},
        ymode = log,
        xmin = 0,
        xmax = 20,
        log ticks with fixed point,
        yminorticks = false,
        tick align = outside,
    ]
        \addplot[smooth, color = black, dashed, thick, no markers] table[x index = 1, y index = 2, col sep = tab] {results/kitchen_metropolis.txt};
        \addplot[smooth, color = red, thick, no markers] table[x index = 1, y index = 2, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla.txt};
        %\addlegendentry{Baseline}
        %\addlegendentry{Ours}
    \end{axis}
\end{tikzpicture}
\clearpage
\begin{tikzpicture}%[scale = .48]
    \begin{axis}[
        grid = major,
        %xlabel = {Computation time in seconds},
        ylabel = {\Gls{mse}},
        ymode = log,
        xmin = 0,
        xmax = 20,
        log ticks with fixed point,
        yminorticks = false,
        tick align = outside,
    ]
        \addplot[smooth, color = black, dashed, thick, no markers] table[x index = 1, y index = 3, col sep = tab] {results/kitchen_metropolis.txt};
        \addplot[smooth, color = red, thick, no markers] table[x index = 1, y index = 3, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla.txt};
        %\addlegendentry{Baseline}
        %\addlegendentry{Ours}
    \end{axis}
\end{tikzpicture}
\clearpage
\begin{tikzpicture}%[scale = .48]
    \begin{axis}[
        grid = major,
        %xlabel = {Computation time in seconds},
        ylabel = {\Gls{mrse}},
        ymode = log,
        xmin = 0,
        xmax = 20,
        log ticks with fixed point,
        yminorticks = false,
        tick align = outside,
    ]
        \addplot[smooth, color = black, dashed, thick, no markers] table[x index = 1, y index = 4, col sep = tab] {results/kitchen_metropolis.txt};
        \addplot[smooth, color = red, thick, no markers] table[x index = 1, y index = 4, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla.txt};
        %\addlegendentry{Baseline}
        %\addlegendentry{Ours}
    \end{axis}
\end{tikzpicture}
\clearpage
\begin{tikzpicture}%[scale = .48]
    \begin{axis}[
        grid = major,
        %xlabel = {Computation time in seconds},
        ylabel = {\Gls{mape}},
        ymode = log,
        xmin = 0,
        xmax = 20,
        log ticks with fixed point,
        yminorticks = false,
        tick align = outside,
    ]
        \addplot[smooth, color = black, dashed, thick, no markers] table[x index = 1, y index = 5, col sep = tab] {results/kitchen_metropolis.txt};
        \addplot[smooth, color = red, thick, no markers] table[x index = 1, y index = 5, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla.txt};
        %\addlegendentry{Baseline}
        %\addlegendentry{Ours}
    \end{axis}
\end{tikzpicture}
\clearpage
\begin{tikzpicture}%[scale = .48]
    \begin{axis}[
        grid = major,
        xlabel = {Computation time in seconds},
        ylabel = {Empirical variance},
        ymode = log,
        xmin = 0,
        xmax = 20,
        log ticks with fixed point,
        yminorticks = false,
        tick align = outside,
    ]
        \addplot[smooth, color = black, dashed, thick, no markers] table[x index = 1, y index = 6, col sep = tab] {results/kitchen_metropolis.txt};
        \addplot[smooth, color = red, thick, no markers] table[x index = 1, y index = 6, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla.txt};
        %\addlegendentry{Baseline}
        %\addlegendentry{Ours}
    \end{axis}
\end{tikzpicture}

\clearpage

\begin{tikzpicture}
    \begin{axis}[
        hide axis,
        xmin = 0,
        xmax = 1,
        ymin = 0,
        ymax = 1,
        legend columns=4,
        legend style = {draw = none, font = \footnotesize, /tikz/every even column/.append style = {column sep = .5cm}},
    ]
        \addlegendimage{black, dashed, thick}
        \addlegendentry{Baseline}
        \addlegendimage{red, thick}
        \addlegendentry{Ours}
    \end{axis}
\end{tikzpicture}

% \clearpage

% \begin{tikzpicture}%[scale = .48]
%     \begin{axis}[
%         title = {\textsc{Country Kitchen}},
%         % title style = {yshift = -1.5ex},
%         grid = major,
%         xlabel = {\Gls{spp}},
%         ylabel = {\Gls{mse}},
%         ymode = log,
%         xmin = 0,
%         xmax = 100,
%         log ticks with fixed point,
%         xtick = {10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
%         xticklabels = {$10$, $20$, $30$, $40$, $50$, $60$, $70$, $80$, $90$, $100$},
%         ytick = {.1, .25, .5, 1},
%         yticklabels = {$.1$, $.25$, $.5$, $1$},
%         yminorticks = false,
%         tick align = outside,
%     ]
%         \addplot[smooth, color = black, dashed, thick, no markers] table[x index = 0, y index = 3, col sep = tab] {results/kitchen_Metropolis\_Restore.txt};
%         \addplot[smooth, color = red, thick, no markers] table[x index = 0, y index = 3, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla.txt};
%         \addplot[smooth, color = blue, thick, no markers] table[x index = 0, y index = 3, col sep = tab] {results/kitchen_Metropolis\_Restore_waste_recycling.txt};
%         \addlegendentry{Restore}
%         \addlegendentry{Restore Vanilla}
%         \addlegendentry{Restore WR}
%     \end{axis}
% \end{tikzpicture}

% \clearpage

% \begin{tikzpicture}%[scale = .48]
%     \begin{axis}[
%         title = {\textsc{Country Kitchen}},
%         % title style = {yshift = -1.5ex},
%         grid = major,
%         xlabel = {\Gls{spp}},
%         ylabel = {Empirical variance},
%         ymode = log,
%         xmin = 0,
%         xmax = 100,
%         log ticks with fixed point,
%         xtick = {10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
%         xticklabels = {$10$, $20$, $30$, $40$, $50$, $60$, $70$, $80$, $90$, $100$},
%         ytick = {.1, .25, .5, 1},
%         yticklabels = {$.1$, $.25$, $.5$, $1$},
%         yminorticks = false,
%         tick align = outside,
%     ]
%         \addplot[smooth, color = black, dashed, thick, no markers] table[x index = 0, y index = 6, col sep = tab] {results/kitchen_Metropolis\_Restore.txt};
%         \addplot[smooth, color = red, thick, no markers] table[x index = 0, y index = 6, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla.txt};
%         \addplot[smooth, color = blue, thick, no markers] table[x index = 0, y index = 6, col sep = tab] {results/kitchen_Metropolis\_Restore_waste_recycling.txt};
%         \addlegendentry{Restore}
%         \addlegendentry{Restore Vanilla}
%         \addlegendentry{Restore WR}
%     \end{axis}
% \end{tikzpicture}

% \clearpage

% \begin{tikzpicture}%[scale = .48]
%     \begin{axis}[
%         title = {\textsc{Country Kitchen}},
%         % title style = {yshift = -1.5ex},
%         grid = major,
%         xlabel = {Rendering time in seconds},
%         ylabel = {\Gls{mse}},
%         ymode = log,
%         xmin = 0,
%         xmax = 20,
%         log ticks with fixed point,
%         xtick = {5, 10, 15, 20},
%         xticklabels = {$5$, $10$, $15$, $20$},
%         ytick = {.1, .25, .5, 1},
%         yticklabels = {$.1$, $.25$, $.5$, $1$},
%         yminorticks = false,
%         tick align = outside,
%     ]
%         \addplot[smooth, color = black, dashed, thick, no markers] table[x index = 1, y index = 3, col sep = tab] {results/kitchen_Metropolis\_Restore.txt};
%         \addplot[smooth, color = red, thick, no markers] table[x index = 1, y index = 3, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla.txt};
%         \addplot[smooth, color = blue, thick, no markers] table[x index = 1, y index = 3, col sep = tab] {results/kitchen_Metropolis\_Restore_waste_recycling.txt};
%         \addlegendentry{Restore}
%         \addlegendentry{Restore Vanilla}
%         \addlegendentry{Restore WR}
%     \end{axis}
% \end{tikzpicture}

% \clearpage

% \begin{tikzpicture}%[scale = .48]
%     \begin{axis}[
%         title = {\textsc{Country Kitchen}},
%         % title style = {yshift = -1.5ex},
%         grid = major,
%         xlabel = {Rendering time in seconds},
%         ylabel = {Empirical variance},
%         ymode = log,
%         xmin = 0,
%         xmax = 20,
%         log ticks with fixed point,
%         xtick = {5, 10, 15, 20},
%         xticklabels = {$5$, $10$, $15$, $20$},
%         ytick = {.1, .25, .5, 1},
%         yticklabels = {$.1$, $.25$, $.5$, $1$},
%         yminorticks = false,
%         tick align = outside,
%     ]
%         \addplot[smooth, color = black, dashed, thick, no markers] table[x index = 0, y index = 6, col sep = tab] {results/kitchen_Metropolis\_Restore.txt};
%         \addplot[smooth, color = red, thick, no markers] table[x index = 1, y index = 6, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla.txt};
%         \addplot[smooth, color = blue, thick, no markers] table[x index = 1, y index = 6, col sep = tab] {results/kitchen_Metropolis\_Restore_waste_recycling.txt};
%         \addlegendentry{Restore}
%         \addlegendentry{Restore Vanilla}
%         \addlegendentry{Restore WR}
%     \end{axis}
% \end{tikzpicture}

% \clearpage

% \begin{tikzpicture}%[scale = .48]
%     \begin{axis}[
%         title = {\textsc{Country Kitchen}},
%         % title style = {yshift = -1.5ex},
%         grid = major,
%         xlabel = {\Gls{spp}},
%         ylabel = {\Gls{mse}},
%         ymode = log,
%         xmin = 0,
%         xmax = 100,
%         log ticks with fixed point,
%         xtick = {10, 20, 30, 40, 50, 60, 70, 80, 90, 100},
%         xticklabels = {$10$, $20$, $30$, $40$, $50$, $60$, $70$, $80$, $90$, $100$},
%         ytick = {.1, .25, .5, 1},
%         yticklabels = {$.1$, $.25$, $.5$, $1$},
%         yminorticks = false,
%         tick align = outside,
%     ]
%         \addplot[smooth, color = black, dashed, thick, no markers] table[x index = 1, y index = 3, col sep = tab] {results/kitchen_metropolis_vanilla.txt};
%         \addplot[smooth, color = red, thick, no markers] table[x index = 1, y index = 3, col sep = tab] {results/kitchen_Metropolis\_Restore_vanilla.txt};
%         \addlegendentry{Metropolis Vanilla}
%         \addlegendentry{Restore Vanilla}
%     \end{axis}
% \end{tikzpicture}

